On Systematic Testing for Execution-Time Analysis

Given a program and a time deadline, does the program finish before the deadline when executed on a given platform? With the requirement to produce a test case when such a violation can occur, we refer to this problem as the worst-case execution-time testing (WCETT) problem. In this paper, we present an approach for solving the WCETT problem for loop-free programs by timing the execution of a program on a small number of carefully calculated inputs. We then create a sequence of integer linear programs the solutions of which encode the best timing model consistent with the measurements. By solving the programs we can find the worst-case input as well as estimate execution time of any other input. Our solution is more accurate than previous approaches and, unlikely previous work, by increasing the number of measurements we can produce WCETT bounds up to any desired accuracy. Timing of a program depends on the properties of the platform it executes on. We further show how our approach can be used to quantify the timing repeatability of the underlying platform.

==> macros.tex <==
\newcommand{\comment}[1]{}
\newcommand{\etal}{{\it et al.}}

\newcommand{\draftRemark}[1]{{\bf{[TODO:#1]}}}

%%% This macro needs the package ``rotating''
\newcommand{\printSideWays}[1]{{\begin{sideways}#1\end{sideways}}}

%% Get .eps or other figure file from subdirectory
\newcommand{\findfigure}[1]{figures/#1}

%% My version of captions
\newcommand{\mycaption}[2]{\caption[#1]{{\bf #1} {{\normalfont{\footnotesize #2}}}}}
%\newcommand{\mycaption}[2]{\caption[#1]{{\bf #1} {{\normalfont{\small #2}}}}}

\setlength{\parskip}{1ex}
\setlength{\parindent}{0em}


\newcommand{\smvertspace}{}
\newcommand{\medvertspace}{}
\newcommand{\bigvertspace}{}

%%%%%%%%%%% For centering table entries on decimal point %%%%%%%%%%%%%%%%%%
%\newcolumntype{.}{D{.}{.}{-1}}
%\newcolumntype{i}{D{.}{.}{2}} % useful for integers, specifying arbit #dec. places causes too wide a colum

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{conjecture}{Conjecture}
\newtheorem{definition}{Definition}

%% Proof stuff
%\newcommand{\qed}{\mbox{} $\Box$}
%\newenvironment{proof}{{\it Proof:}}{\qed}


%%%%%%% General math and algos stuff %%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Reals}{\ensuremath{\mathbb{R}}}
\newcommand{\Integers}{\ensuremath{\mathbb{Z}}}
\newcommand{\Naturals}{\ensuremath{\mathbb{N}}}

\newcommand{\BigOh}{\ensuremath{\mathcal{O}}}
\newcommand{\Algo}{\ensuremath{\mathcal{A}}}


\newcommand{\bnf}{\mathrel{::=}}
\newcommand{\kw}[1]{{\bf #1}}
\newcommand{\sk}[1]{{\sf #1}}
\newcommand{\va}[1]{{\rm {\it #1}}}
\newcommand{\mva}[1]{\mbox{\va{#1}}}
%%\newcommand{\syntaxform}[1]{\langle \mva{#1} \rangle}
\newcommand{\syntaxform}[1]{\mva{#1}}
\newcommand{\vbar}{\mathbin{|}}
\newcommand{\lvbar}{|\;}

\newcommand{\mktt}[1]{{\tt{#1}}}

\newcommand{\mkttt}[1]{{$\mktt{#1}$}}


\newcommand{\stmt}{\ensuremath{S}}
\newcommand{\intstmt}{\ensuremath{R}}
\newcommand{\task}{\ensuremath{T}}
\newcommand{\pgm}{\ensuremath{P}}
\newcommand{\seq}{\ensuremath{P_{\text{seq}}}}

\newcommand{\assn}{\ensuremath{:=}}
\newcommand{\upd}{\ensuremath{\leftarrow}}

\newcommand{\gametime}{{\sc{GameTime}}\xspace}

\newcommand{\intr}{\ensuremath{\iota}}
\newcommand{\arr}{\ensuremath{\alpha}}

\newcommand{\cb}{\ensuremath{\mathit{CB}}}
%\newcommand{\cs}{\ensuremath{\nu_{\text{cs}}}}
\newcommand{\cs}{\ensuremath{C}}


\newcommand{\Path}{\ensuremath{\boldsymbol{x}}}
\newcommand{\Pathy}{\ensuremath{\boldsymbol{y}}}
\newcommand{\basis}[1][i]{\ensuremath{\boldsymbol{b}_{#1}}}
\newcommand{\Pathopt}{\ensuremath{\Path^*}}
\newcommand{\Paths}{\ensuremath{\mathcal P}}
\newcommand{\PathsSub}{\ensuremath{\mathcal P}_{\text{sub}}}
\newcommand{\weight}[1][t]{\ensuremath{\boldsymbol{w}_{#1}}}
\newcommand{\estweight}[1][t]{\ensuremath{\tilde{\boldsymbol{w}}_{#1}}}
\newcommand{\basisweight}[1][t]{\ensuremath{\boldsymbol{v}_{#1}}}
\newcommand{\estbasisweight}[1][t]{\ensuremath{\tilde{\boldsymbol{v}}_{#1}}}

\newcommand{\pertvector}{\ensuremath{{\boldsymbol{\pi}}}}
\newcommand{\pertvec}{\ensuremath{{{\boldsymbol{\pi}}^{\Path}}}}
\newcommand{\pert}{\ensuremath{\boldsymbol{p}}}

\newcommand{\E}{\ensuremath{\mathbb E}}
\newcommand{\R}{\ensuremath{\mathbb R}}
\newcommand{\Sexp}{\ensuremath{\mathcal S}}
\newcommand{\Semp}{\ensuremath{\tilde{\mathcal S}}}
\newcommand{\tr}{\ensuremath{{\scriptscriptstyle\mathsf{T}}}}
\newcommand{\mub}{\ensuremath{\boldsymbol{\mu}}}
\newcommand{\alphab}{\ensuremath{\boldsymbol{\alpha}}}
\newcommand{\mugen}{\ensuremath{{{\boldsymbol{\mu}}^{\Path}}}}

\newcommand{\PathPredicted}[1]{\ensuremath{\boldsymbol{x}^*_{#1}}}

\newcommand{\Len}{\ensuremath{\mathcal{L}}}

\newcommand{\mumax}{\ensuremath{\mu_{\max}}}

\newcommand{\pimax}{\ensuremath{\pi_{\max}}}

\newcommand{\sigmadiff}{\ensuremath{\sigma_{\text{diff}}}}

\newcommand{\wdiff}{\ensuremath{w_{\text{diff}}}}

%%%%%%%%%%%%%%% Software related %%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\lab}[1]{\protect\label{#1}}

\newcommand{\sil}{{\sc sil}\xspace}


\newcommand{\hbra}{
\hbox to \textwidth{\vrule width0.3mm height 1.8mm depth-0.3mm
                    \leaders\hrule height1.8mm depth-1.5mm\hfill
                    \vrule width0.3mm height 1.8mm depth-0.3mm}}
\newcommand{\hket}{
\hbox to \textwidth{\vrule width0.3mm height1.5mm
                    \leaders\hrule height0.3mm\hfill
                    \vrule width0.3mm height1.5mm}}


\renewcommand{\hbra}{
\hbox to \columnwidth{\vrule width0.3mm height 1.8mm depth-0.3mm
                    \leaders\hrule height1.8mm depth-1.5mm\hfill
                    \vrule width0.3mm height 1.8mm depth-0.3mm}}
\renewcommand{\hket}{
\hbox to \columnwidth{\vrule width0.3mm height1.5mm
                    \leaders\hrule height0.3mm\hfill
                    \vrule width0.3mm height1.5mm}}



\newsavebox{\DispFigName}
\newenvironment{displayfig}[1]{
  \refstepcounter{figure}
  \begin{figure}[h]
  \hbra
%  \hbra\\[-.8ex]
  \sbox{\DispFigName}{#1}
  }{
  \\\hket
%  \\[-.8ex]\hket
   \center{Figure \thefigure: {\usebox{\DispFigName}}}
  \end{figure}
}





%%%%%%%%%%%%%%%%%%%%% MISC %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Space saving List environment for enumerations.
\newcounter{myctr}
\newenvironment{mylist}{\begin{list}{\arabic{myctr}.}
{\usecounter{myctr}
\setlength{\topsep}{1mm}\setlength{\itemsep}{0.25mm}
\setlength{\parsep}{0.1mm}
\setlength{\itemindent}{0mm}\setlength{\partopsep}{0mm}
\setlength{\labelwidth}{15mm}
\setlength{\leftmargin}{4mm}}}{\end{list}}

% Space saving List environment for itemizing
\newenvironment{myitemize}{\begin{list}{$\bullet$}
{\setlength{\topsep}{1mm}\setlength{\itemsep}{0.25mm}
\setlength{\parsep}{0.1mm}
\setlength{\itemindent}{0mm}\setlength{\partopsep}{0mm}
\setlength{\labelwidth}{15mm}
\setlength{\leftmargin}{4mm}}}{\end{list}}



